Sequential Functional Structured Tucker Compression for Large Language Model Attentions

Post-training compression of LLM attention is often formulated as independent matrix approximation, ignoring both the shared structure among attention projections and the representation shift introduced by earlier compression. We propose FTC, a sequential structured compression framework that adapts the approximation to the current compressed model while jointly exploiting the native Q/K/V head structure under a fixed storage budget. The output projection is handled separately to account for the changed post-attention representation. FTC requires neither fine-tuning nor gradient-based recovery. Across seven decoder-only LLMs from 6B to 32B parameters, FTC achieves the lowest WikiText-2 perplexity among the compared methods at every tested keep ratio on five modern GQA models, with the largest gains under aggressive compression. The improvements transfer to downstream tasks and remain substantial at the 32B scale.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

\usepackage{xcolor}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Setup}
\label{sec:setup}

\paragraph{Models.}
We evaluate on seven decoder-only LLMs spanning three architectural
generations: the MHA trio used by LeSTD --- GPT-J-6B, Llama-2-13B, and
OPT-30B --- and four modern GQA models --- Mistral-7B-v0.3, Llama-3-8B,
Qwen2.5-7B, and Qwen3-8B-Base (the latter with QK-norm).
Section~\ref{sec:hybrid} additionally extends the method to Qwen3.5-9B-Base,
a hybrid architecture in which 24 of 32 layers use GatedDeltaNet linear
attention and the remaining 8 use gated GQA.

\paragraph{Baselines.}
Six methods run under one protocol: \ftc{} (ours); \textbf{enh-LeSTD}, our
head-concat port of LeSTD to GQA (on MHA models we report native LeSTD, which
is otherwise undefined on grouped heads); \textbf{TLLM-gen}, a
TensorLLM-style data-free dense Tucker factorization; \textbf{MPIFA};
\textbf{SVD-LLM}; and \textbf{Basis Sharing}. SliceGPT compresses the hidden
dimension rather than the attention projections and is compared separately
under whole-model accounting in Appendix~\ref{app:e2e}.

\paragraph{Protocol.}
\ftc{} uses 256 calibration sequences of 2{,}048 tokens from WikiText-2
train (seed 42); the data-dependent baselines use the 128 sequences of their
published configurations, and Table~\ref{tab:calibsize} shows what \ftc{}
loses at 128 so the reader can price that difference. All methods share the
same evaluation windows and the same parameter accounting: the compression ratio
$\rrho$ is the \emph{kept} fraction of attention-projection parameters
(LeSTD's convention), so smaller $\rrho$ means stronger compression. The sparse core's index is
charged against that budget, so $\rrho$ is what the compressed model
actually stores and the \ftc{} column is directly comparable to the
low-rank baselines, which have no index; attention projections are 11--33\%
of the whole model, so e.g.\ Llama-3-8B at $\rrho{=}0.2$ is a 13\%
whole-model reduction --- the exact accounting per cell is in
Appendix~\ref{app:accounting}. Compressing the FFN as well is checked on one
model (Appendix~\ref{app:e2e}); the claims in this section are about the
attention projections.
The \ftc{} recipe is fixed across all models and ratios (allocator
$\beta{=}0.5$, anchor $a{=}0.5$, no teacher map on the QKV tensor, $W_O$
compressed under its own attention-output metric with the closed-form
teacher map at $\mu{=}1$, $\alpha{=}0.02$, two refits, 256 calibration
windows, slab-norm); Table~\ref{tab:uniform} reports exactly this recipe
everywhere. During
development we also ran a small set of variants (the QKV teacher map at
$\mu\in\{0.1,0.3,1,3,10\}$, anchor auto, $\beta\in\{0.35,0.65\}$,
128/384 windows); those appear only in the ablations of
Section~\ref{sec:ablation} and Appendix~\ref{app:hyper}, never in a main
table, so every \ftc{} cell reported below is the one recipe and baselines
run their published configuration. The
whole pipeline is deterministic: re-running any cell reproduces perplexity to
three decimals, and cells where the rotation guard is inactive reproduce
bit-identically. No fine-tuning or gradient-based recovery is used anywhere.


\subsection{Main results: perplexity across three model generations}
\label{sec:main-results}

\begin{table}[t]
\centering\small
\caption{WikiText-2 perplexity at $\rrho\in\{0.6,0.2\}$ (dense ppl in
parentheses; best per row in bold). Every cell is compressed to the same
realised $\rrho$ \emph{including} the sparse-core index, so the columns are
directly comparable (Appendix~\ref{app:accounting}).
\textbf{Seq-SVD is not a published method}: it is our own ``no joint
tensor'' ablation, i.e.\ per-matrix functional SVD under the same whitened
metric and the same sequential dual-stream calibration as \ftc{}, printed
here as the strongest per-matrix control we can build. The enh-LeSTD column
is native LeSTD where it runs (GPT-J at $\rrho\ge0.6$) and our GQA-capable
reimplementation elsewhere, including GPT-J at $\rrho{=}0.2$ where native
LeSTD diverges (Appendix~\ref{app:protocol}). SVD-LLM V2 (Wang et al.,
NAACL 2025) has no public implementation; our reproduction of its
Algorithms 1--2 matches SVD-LLM at $\rrho{=}0.6$ but its heterogeneous
rank allocation degenerates at $\rrho{=}0.2$, so we report SVD-LLM only
and document the attempt in Appendix~\ref{app:svdllmv2}.
\ftc{} cells are the single fixed recipe of Section~\ref{sec:setup}.
Calibration-seed variance (three seeds, every GQA model, all four ratios)
is at most $\pm0.03$ ppl for \ftc{} and at most $\pm0.05$ for enh-LeSTD at
$\rrho{\ge}0.6$; every \ftc{} margin at $\rrho{\le}0.6$ is at least $23$
seed-standard-deviations wide. The one exception is Llama-3-8B at
$\rrho{=}0.8$, a tie with enh-LeSTD ($6.36$ vs.\ $6.36$)
(Appendix~\ref{app:uniform}). Full four-ratio sweeps and PTB/C4 are in
Appendix~\ref{app:full-ppl}.}
\label{tab:main}
\setlength{\tabcolsep}{3pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llc|ccccc c}
\toprule
& & & \multicolumn{6}{c}{per-matrix factorizations}\\
\cmidrule(l){4-9}
Model & $\rrho$ & \ftc{} & Seq-SVD & enh-LeSTD & TLLM-gen & MPIFA & SVD-LLM & Basis \\
\midrule
\primitiveinput tables/t1_main_ppl.tex 
\bottomrule
\end{tabular}}
\end{table}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/f1_ratio_sweep.pdf}
\caption{Perplexity vs.\ keep ratio for all seven models (log scale; dotted
line = dense). \ftc{} is lowest in every modern-model cell at every ratio,
and its margin widens monotonically with compression strength.}
\label{fig:sweep}
\end{figure}

Table~\ref{tab:main} and Figure~\ref{fig:sweep} give the headline result.
Three observations:

\textbf{(1) The margin grows with compression strength and architectural
modernity.} At $\rrho{=}0.8$ on MHA models all reasonable methods are within
a few percent of dense and enh-LeSTD is occasionally best (we report this
faithfully). By $\rrho{=}0.2$ on modern GQA models the field collapses ---
SVD-LLM reaches 4.8--37$\times$ dense ppl, MPIFA blows up on Qwen2.5 --- while
\ftc{} stays at 1.3--1.7$\times$ dense on three of four models (Qwen2.5-7B is
the exception at 3.5$\times$; Appendix~\ref{app:protocol} explains why its whitening metric degrades at this budget). Across the 16
modern-model cells \ftc{} is best in all 16, with a 39--88\% ppl advantage over the runner-up at $\rrho{=}0.2$.

\textbf{(1b) What the Seq-SVD column is for.} A reader is entitled to ask
how much of that margin is the objective --- the whitened functional metric
and the sequential dual-stream calibration --- and how much is the joint
tensor, since the objective can be bolted onto any per-matrix method. The
Seq-SVD column answers it directly: it \emph{is} our objective, applied to
per-matrix SVD, and it is the strongest per-matrix control we can construct.
It lands squarely in the published per-matrix band rather than above it: at
$\rrho{=}0.2$ it beats every published per-matrix method on Mistral-7B
($12.10$ vs.\ $15.92$) and Llama-3-8B ($19.46$ vs.\ $20.84$), and loses to
the best one on Qwen2.5-7B ($150.93$ vs.\ $106.59$) and Qwen3-8B ($23.66$
vs.\ $22.23$). So the objective alone buys a per-matrix method roughly what
the best-tuned per-matrix methods already have; the separation to $7.14$,
$10.21$, $12.55$ and $10.60$ is the joint tensor. We say this rather than
letting the ablation grid imply that any one ingredient carries the result.

\textbf{(2) The three-generation ordering holds in 15 of 16 modern cells.}
TLLM-gen $<$ enh-LeSTD $<$ \ftc{} in quality: joint head structure helps,
sparse-core annealing on top helps, and the functional metric on top helps
again. The one exception is Mistral-7B at $\rrho{=}0.2$, where enh-LeSTD
itself collapses (146.3) and falls behind TLLM-gen (18.4) --- \ftc{} is still
best in that cell by a wide margin. This compositional evidence is the
experimental backbone of the attribution study in
Section~\ref{sec:ablation}.

\textbf{(3) The result survives a $4\times$ scale-up, but the margin
narrows.} Qwen3-32B is the same architecture family as Qwen3-8B --- GQA
$64/8$, QK-norm, $64$ layers --- at four times the parameters, so it
isolates scale from every other axis. It is compressed one decoder layer at
a time on a single 40GB card with the weights on CPU, under the identical
recipe and accounting, against the same six baselines. Against a dense
perplexity of $7.61$, \ftc{} is best in every cell: $7.65$ at $\rrho{=}0.8$
and $9.22$ at $\rrho{=}0.2$ ($1.21\times$ dense).

The honest reading of the comparison is that scale helps the strongest
baseline more than it helps us. At $\rrho{=}0.2$ \ftc{} is $2.08\times$
better than the best baseline on Qwen3-8B (MPIFA, $22.23$) and
$1.65\times$ better on Qwen3-32B (enh-LeSTD, $15.23$); at $\rrho{=}0.8$ the
$32$B cell is a tie ($7.65$ against enh-LeSTD's $7.66$). We report this
rather than the number we would get by quoting MPIFA at both scales, which
would have read as a widening margin.

\subsection{Downstream tasks}
\label{sec:downstream}

\begin{table}[t]
\centering\small
\caption{Downstream accuracy at $\rrho\in\{0.6,0.4,0.2\}$ on the modern GQA
models: per method we report avg6 (mean acc\_norm over PIQA, ARC-e, ARC-c,
HellaSwag, WinoGrande, LAMBADA) and 5-shot GSM8K accuracy. Dense (avg6 /
GSM8K) in the row label. \ftc{} cells are the single fixed recipe of
Section~\ref{sec:setup}; baselines run their published configuration. GSM8K
\emph{is} reported at $\rrho{=}0.2$, but no winner is marked there: on the
7--8B models every method, \ftc{} included, scores $0.00$--$0.03$, i.e.\ at
or below chance for a 5-shot exact-match task, and bolding a winner would be
bolding noise. Qwen3-32B is the one exception --- \ftc{} keeps $0.28$ while
every baseline is at $0.00$--$0.01$ --- and we leave it unmarked for
consistency rather than mark a single row
(Section~\ref{sec:drift}). The complete per-task grid --- all methods, all four
ratios, MathQA included, plus the MHA models and the development variants ---
is in Appendix~\ref{app:full-tasks}.}
\label{tab:downstream}
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llcc|cccccccccccc}
\toprule
& & \multicolumn{2}{c|}{\ftc{}} & \multicolumn{2}{c}{Seq-SVD} & \multicolumn{2}{c}{enh-LeSTD}
& \multicolumn{2}{c}{TLLM-gen} & \multicolumn{2}{c}{MPIFA}
& \multicolumn{2}{c}{SVD-LLM} & \multicolumn{2}{c}{Basis} \\
Model & $\rrho$ & a6 & G8K & a6 & G8K & a6 & G8K & a6 & G8K & a6 & G8K & a6 & G8K & a6 & G8K \\
\midrule
\primitiveinput tables/t2_downstream.tex 
\bottomrule
\end{tabular}}
\end{table}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/f3_downstream.pdf}
\caption{Downstream retention vs.\ kept fraction on the four GQA models
(\ftc{} = fixed final recipe, thick red). Top: avg6 relative to dense.
Bottom: 5-shot GSM8K relative to dense; the dashed line is 10\% retention.
The $\rrho{=}0.2$ point is drawn but is at or below chance for every method
(Table~\ref{tab:downstream}). \ftc{} is the only method whose GSM8K curve is
still above the line at $\rrho{=}0.4$ on every model.}
\label{fig:downstream}
\end{figure}

Perplexity advantages transfer to tasks (Table~\ref{tab:downstream}, Figure~\ref{fig:downstream}), and
\ftc{} holds the best avg6 in every cell, and the best GSM8K in every cell
at $\rrho\ge0.4$. At $\rrho{=}0.2$ GSM8K stops discriminating: every method
including ours scores $0.00$--$0.03$ on the 200 problems, i.e.\ at or below
chance for a 5-shot exact-match task, so we report the column but mark no
winner in it. Three patterns
matter. First, \emph{decay slopes differ by generation}: from $\rrho{=}0.8$
to $0.4$, \ftc{} loses $4$--$11$ avg6 points (Llama-3 $.729\!\to\!.670$)
where enh-LeSTD loses $10$--$21$ and SVD-LLM $20$--$29$. Second,
\emph{generative reasoning is the canary}: GSM8K decays far earlier than the
multiple-choice average --- at $\rrho{=}0.6$ on Qwen3-8B, \ftc{} retains
$.710/.855=83\%$ of dense GSM8K while SVD-LLM retains $23\%$ --- and at
$\rrho{=}0.4$ \ftc{} is the only method that keeps more than a fifth of dense
GSM8K on any model ($33\%$, $25\%$, $56\%$, $18\%$ on the four models
against at most $11\%$ for the best baseline), which motivates the drift
analysis below. Third, at $\rrho{=}0.2$, where reasoning is gone for every
method, the multiple-choice margin is at its widest on the three models that
still function: \ftc{} leads the best baseline by $14$--$18$ avg6 points on
Mistral-7B, Llama-3-8B and Qwen3-8B, and by $3$ points on Qwen2.5-7B, where
every method including ours has collapsed to near the task floor.

\subsection{Attribution and ablations}
\label{sec:ablation}

\begin{table}[t]
\centering\scriptsize
\caption{Component attribution. ``full'' is the final recipe of
Section~\ref{sec:setup}; every column removes exactly one ingredient from it
and reports WikiText-2 ppl with the relative change, both arms compressed to
the same realised ratio. ``w/o whitening'' replaces the functional metric by
the identity, ``w/o slab-norm'' drops the per-head-slot energy
normalisation, ``w/o seq.\ calibration'' takes every Gram from the teacher
stream instead of the compressed one, ``K/V repeat-expand'' replaces the
head-concat tensor by the naive GQA$\to$MHA tensorization, ``dense core''
keeps the whitened factors but uses a dense core of matched size, ``no joint
tensor'' factorizes $W_Q,W_K,W_V$ separately under the same metric, and
``w/o $W_O$ target'' drops the closed-form teacher target on the output
projection. Every cell is compressed under the index-cost accounting of
Appendix~\ref{app:accounting} and scored against the reference built the
same way: the six columns that leave the tensorization free run with
per-layer layout selection and are scored against the full recipe with it
on, while ``K/V repeat-expand'' and ``no joint tensor'' cannot use it and
are scored against the full recipe with the layout pinned to head-concat.
The two references coincide wherever layout selection picks head-concat on
every layer, and separate where it does not --- on Qwen2.5-7B at
$\rrho{=}0.2$ they are $12.55$ and $22.04$.}
\label{tab:ablation}
\setlength{\tabcolsep}{3pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
\primitiveinput tables/abl_grid_hdr.tex 
\midrule
\primitiveinput tables/abl_grid.tex 
\bottomrule
\end{tabular}}
\end{table}

Table~\ref{tab:ablation} removes one ingredient at a time from the final
recipe, both arms compressed to the same realised ratio. Two things hold
across the whole grid: at $\rrho{=}0.6$ every ingredient is worth at most a
few percent, and at $\rrho{=}0.2$ the same ingredients are worth tens to
hundreds of percent, so the recipe is a statement about aggressive budgets.

\emph{Sequential calibration} --- taking every Gram from the compressed
stream rather than from the original model --- costs $+25$ to $+451\%$ at
$\rrho{=}0.2$, and is the largest single ingredient on Qwen3-8B ($+451\%$)
and Llama-3-8B ($+226\%$). It is smallest on Qwen2.5-7B ($+25\%$), the model
already furthest from dense at this budget, which is what one expects if its
value is that the metric tracks a stream still worth tracking. Anchoring half
of the $W_O$ statistics to the teacher Gram is a separate and much smaller
refinement ($+3$ to $+19\%$, within $\pm1\%$ at $\rrho{=}0.6$).

Three structural choices carry the rest. \emph{Whitening} costs $+79$ to
$+748\%$: the un-whitened Tucker fit spends its budget on directions the
input never excites. The \emph{joint head-concat tensor} costs $+69$ to
$+522\%$: factorizing $W_Q,W_K,W_V$ separately under the same functional
metric loses the shared head structure. \emph{Slab-norm} --- equalising the
whitened energy of each head slot so no slot monopolises the shared bases and
the core budget --- costs $+10.5$ to $+160.8\%$. Its ordering is instructive:
Qwen3-8B is the one QK-normalized model here and it benefits \emph{least},
so this is a stabiliser for tight budgets rather than a fix for unconstrained
$q/k$ scales. The annealed \emph{sparse core}
is worth a consistent $+7$ to $+12\%$ over a dense core of matched size.

Two results are conditional on the architecture. The head-concat
tensorization beats the naive GQA$\to$MHA repeat-expand by $+48$, $+49$ and
$+77\%$ on Mistral-7B, Qwen3-8B and Llama-3-8B, all of which have four query
heads per K/V head, but \emph{loses} to it by $50\%$ on Qwen2.5-7B, which has
seven: folding K and V into four shared slots evidently discards more there
than the shared basis saves, and expanding to full width buys each K/V head
its own core entries at the same parameter budget. The blow-up counter of
Table~\ref{tab:escalation} tracks the sign exactly: where repeat-expand
loses it destabilises $16$--$22$ layers (five to seven of them all the way to
$\varepsilon{=}1$), and on Qwen2.5-7B, where it wins, it destabilises none
--- while the head-concat arm there destabilises nine. The layout that fits
the better-conditioned joint tensor is the one that wins, and which layout
that is depends on the K/V sharing factor. We report the head-concat
tensorization as the recipe because it wins on three of four models and never
costs parameters, but on a $7{:}1$ GQA model at $\rrho{=}0.2$ it is the wrong
structure by a factor of two ($24.26$ against $12.12$ at a realised $0.200$
in both arms), and we do not claim it as universal. Likewise the closed-form
\emph{teacher target} on $W_O$ is worth $+41$, $+42$ and $+191\%$ on those
same three models and a $29\%$ \emph{loss} on Qwen2.5-7B, whose student and
teacher streams have decorrelated by this budget. Applying that target to
$Q/K/V$ instead is harmful everywhere at $\rrho{=}0.2$ ($+3.5$ to $+34.2\%$)
and neutral at $\rrho\ge0.4$, which is why the recipe uses a static target
there.

The $\mu$ sweep in
Appendix~\ref{app:hyper} approaches the same conclusion from the other side:
$\mu$ interpolates between regressing on the teacher stream and the static
target, and on every model the static end is best, with the largest single
step being the last one. That is why the final recipe fits the QKV tensor to
the LeSTD-style static target under our whitened metric and sparse core, and
keeps a teacher map only on $W_O$, whose input is the attention output that
upstream compression has already perturbed.
Appendix~\ref{app:hyper} reports the remaining knobs (refit count, anchor,
calibration size, allocator $\beta$, and the damping of the whitening
metric).

\paragraph{Sparsity-aligned rotation.}
The gauge freedom of the Tucker core admits an orthogonal warm-start that
rotates energy into the surviving sparsity pattern before annealing. Its
value obeys a simple law: \emph{gain $\approx$ constraint hardness $\times$
core energy headroom}. Most whitened GQA cores are already 99.6--99.9\%
top-$K$-saturated, so a guard (apply only if the rotation buys
$>\tau{=}0.005$ top-$K$ energy) makes it a no-op on Llama-3-8B, Mistral-7B
and Qwen3-8B, whose cells are then bit-identical with the rotation disabled;
it does fire on Qwen2.5-7B, whose cores are the least saturated of the four
($11$ of $28$ layers at $\rrho{=}0.2$, $16$ of $28$ at $\rrho{=}0.4$). On MHA
cores with headroom it fires and helps
slightly (GPT-J: $9.26\!\to\!9.24$ at $\rrho{=}0.6$), and under hard 2:4
structure it helps a lot ($21.9\!\to\!18.9$ at $\rrho{=}0.2$,
a $-13.6\%$ ``pattern tax'' rebate). The rotation is default-on with the
guard in all reported \ftc{} numbers; the full archive is in
Appendix~\ref{app:rotation}.

\subsection{Why it works: functional drift predicts task survival}
\label{sec:drift}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/f2_drift_task.pdf}
\caption{Last-layer functional drift vs.\ task retention and perplexity over
every compressed GQA model with a task row ($n{=}136$: 4 models, 6 methods,
4 ratios, plus the \ftc{} recipe variants of Appendix~\ref{app:hyper}).
Drift predicts avg6 retention with Pearson $-0.89$ / Spearman $-0.92$ and
GSM8K retention with $-0.73$ / $-0.90$; per model the Spearman coefficients
range from $-0.80$ to $-0.98$ (avg6). Drift and WikiText-2 perplexity are far
from interchangeable (Pearson $0.30$), and perplexity itself predicts avg6
retention with Pearson only $-0.19$ (Spearman $-0.86$): the extreme cells
that dominate a linear fit are exactly where drift keeps its resolution.
GSM8K retention collapses once drift passes ${\approx}0.40$ (dashed line).}
\label{fig:drift}
\end{figure}

Figure~\ref{fig:drift} makes the mechanism explicit: last-layer stream drift
--- exactly the quantity the functional metric minimizes --- predicts
downstream retention across all 136 compressed models (Spearman $-0.92$ for
avg6, $-0.90$ for GSM8K), and GSM8K retention falls off a cliff once drift
exceeds ${\approx}0.40$ (mean retention $.66$ below $0.30$, $.22$ in
$[0.30,0.40)$, $.04$ in $[0.40,0.60)$). The cliff is method-agnostic: at
$\rho{=}0.4$ \ftc{} is the only method left of it on all four models
(drift $0.25$--$0.32$, GSM8K retention $.24$--$.33$), while every baseline
except enh-LeSTD has crossed it and posts GSM8K retention $\le .11$; at
$\rho{=}0.2$ every method, \ftc{} included, is past it and GSM8K is gone for
all of them (Table~\ref{tab:downstream}). Methods that minimize weight-space
error can cross the cliff while still posting moderate perplexity, which is
why the perplexity ordering in Table~\ref{tab:main} understates the
downstream gap; \ftc{} optimizes the predictive quantity directly.
Appendix~\ref{app:depth} shows where along depth this drift accumulates.
\subsection{Extension to hybrid linear-attention architectures}
\label{sec:hybrid}

The head-concat construction requires only that several linear maps share an
input space and split into equal-width output slots. Qwen3.5-9B-Base
satisfies this in both of its layer types: the GatedDeltaNet fused
$W_{\mathrm{qkv}}$ (16 q + 16 k + 32 v heads of width 128, $H{=}64$) and the
gated attention $W_q$ whose output interleaves 16 query heads with 16
gating heads of width 256 ($H{=}40$) --- gates are linear maps of the same
normalized input and compress as ordinary head slots. With \emph{zero
formula changes} (per-layer geometry only), \ftc{} yields:

\begin{center}\small
\begin{tabular}{lccc}
\toprule
 & wt2 ppl & avg6 & GSM8K \\
\midrule
dense & 6.98 & .723 & .885 \\
\ftc{} $\rrho{=}0.8$ & 7.16 (+2.5\%) & .727 (100.5\%) & .785 (89\%) \\
\ftc{} $\rrho{=}0.6$ & 7.68 (+10.0\%) & .690 (95.5\%) & .58 (65\%) \\
\bottomrule
\end{tabular}
\end{center}

The $\rrho{=}0.6$ quality loss (+10.0\%) is \emph{smaller} than on
standard-GQA Qwen3-8B (+13.2\%), all 32 layers compress without a single
guard rollback, and downstream accuracy at $\rrho{=}0.8$ is lossless on
avg6. Per-matrix decomposition baselines on the same architecture are
reported in Appendix~\ref{app:hybrid-anchors}.

\subsection{Deployment}
\label{sec:deploy}

Unstructured sparse cores measure representational limits; deployment needs
structure. Under 2:4 core sparsity with the rotation warm-start, \ftc{} on
GPT-J reaches wt2 9.72 at $\rrho{=}0.6$ (dense-core Tucker: 10.04). Table~\ref{tab:throughput} measures the attention in-projection path on an
idle A100 for all three architecture families, with \emph{both} the dense
baseline and the factorized path given the same three execution modes
(eager, CUDA-graph replay, \texttt{torch.compile} max-autotune) and the
better of the three reported for each side.

Two findings. First, the win at aggressive compression is large and holds
across architectures: $2.53\times$ (MHA), $3.22\times$ (GQA) and
$3.27\times$ (hybrid) at $\rrho{=}0.2$, and $1.05$--$1.82\times$ at
$\rrho{=}0.6$, with GQA and hybrid benefiting most because their narrower
in-projections make the shared factor $U_1$ relatively cheaper. Second,
\emph{how} the kernels are launched dominates at small token counts: the
factor chain issues three kernels where the dense path issues one, so in
eager mode it loses catastrophically at $N{=}1$ ($0.06$--$0.15\times$),
while CUDA-graph replay removes that launch overhead entirely and turns the
same shapes into $1.0$--$1.9\times$ wins at $\rrho{=}0.2$. Deployments that
capture decode steps into graphs --- standard practice in modern serving
stacks --- therefore keep the compression gain in the decode phase; without
graph capture they do not. At the whole-model level the gain is diluted by
the uncompressed FFN (prefill $1.04$--$1.14\times$ on GPT-J), which
end-to-end joint-FFN compression addresses (Appendix~\ref{app:e2e}).

\begin{table}[t]
\centering\small
\caption{Attention in-projection throughput on an idle A100 (fp16,
CUDA-event timing, median of 200). ``best'' compares the fastest execution
mode of the factorized path against the fastest mode of the dense baseline;
``eager'' compares both without graph capture or compilation. $N$ is tokens
per launch ($N{=}64$ stands in for batched decode).}
\label{tab:throughput}
\begin{tabular}{llccc}
\toprule
Architecture & $N$ & $\rrho$ & best & eager \\
\midrule
\primitiveinput tables/t4_throughput.tex 
\bottomrule
\end{tabular}
\end{table}

End-to-end quality (attention+FFN, whole-model accounting) \ftc{} at
$\rrho{=}0.6$ reaches 11.37 vs.\ 15.54 for SVD-LLM end-to-end
(Appendix~\ref{app:e2e}).


==> tables/a3_downstream_full.tex <==
Mistral-7B & dense & 1.0 & 0.814 & 0.807 & 0.530 & 0.796 & 0.740 & 0.753 & 0.367 & 0.285 & 0.740 \\
 & \ftc{} & 0.8 & 0.805 & 0.812 & 0.521 & 0.779 & 0.745 & 0.737 & 0.345 & 0.235 & 0.733 \\
 & \ftc{} & 0.6 & 0.805 & 0.811 & 0.506 & 0.765 & 0.741 & 0.728 & 0.336 & 0.240 & 0.726 \\
 & \ftc{} & 0.4 & 0.795 & 0.781 & 0.474 & 0.726 & 0.701 & 0.655 & 0.303 & 0.105 & 0.689 \\
 & \ftc{} & 0.2 & 0.720 & 0.595 & 0.321 & 0.555 & 0.619 & 0.263 & 0.247 & 0.015 & 0.512 \\
 & Seq-SVD & 0.6 & 0.781 & 0.759 & 0.450 & 0.711 & 0.716 & 0.690 & 0.320 & 0.175 & 0.684 \\
 & Seq-SVD & 0.4 & 0.706 & 0.603 & 0.337 & 0.582 & 0.661 & 0.524 & 0.287 & 0.010 & 0.569 \\
 & Seq-SVD & 0.2 & 0.545 & 0.339 & 0.243 & 0.343 & 0.562 & 0.121 & 0.220 & 0.000 & 0.359 \\
 & enh-LeSTD & 0.8 & 0.805 & 0.807 & 0.509 & 0.774 & 0.736 & 0.738 & 0.345 & 0.260 & 0.728 \\
 & enh-LeSTD & 0.6 & 0.794 & 0.796 & 0.479 & 0.745 & 0.733 & 0.697 & 0.334 & 0.155 & 0.707 \\
 & enh-LeSTD & 0.4 & 0.770 & 0.709 & 0.404 & 0.668 & 0.672 & 0.526 & 0.287 & 0.005 & 0.625 \\
 & enh-LeSTD & 0.2 & 0.524 & 0.300 & 0.252 & 0.295 & 0.535 & 0.011 & 0.213 & 0.000 & 0.320 \\
 & TLLM-gen & 0.8 & 0.798 & 0.790 & 0.484 & 0.748 & 0.725 & 0.711 & 0.331 & 0.190 & 0.709 \\
 & TLLM-gen & 0.6 & 0.770 & 0.738 & 0.426 & 0.699 & 0.695 & 0.594 & 0.314 & 0.095 & 0.654 \\
 & TLLM-gen & 0.4 & 0.694 & 0.540 & 0.320 & 0.552 & 0.632 & 0.270 & 0.242 & 0.010 & 0.501 \\
 & TLLM-gen & 0.2 & 0.566 & 0.337 & 0.259 & 0.335 & 0.537 & 0.016 & 0.209 & 0.015 & 0.342 \\
 & MPIFA & 0.8 & 0.803 & 0.789 & 0.511 & 0.781 & 0.733 & 0.737 & 0.360 & 0.260 & 0.726 \\
 & MPIFA & 0.6 & 0.791 & 0.755 & 0.466 & 0.723 & 0.734 & 0.699 & 0.342 & 0.200 & 0.695 \\
 & MPIFA & 0.4 & 0.710 & 0.581 & 0.320 & 0.539 & 0.653 & 0.508 & 0.276 & 0.020 & 0.552 \\
 & MPIFA & 0.2 & 0.527 & 0.312 & 0.230 & 0.281 & 0.512 & 0.022 & 0.222 & 0.005 & 0.314 \\
 & SVD-LLM & 0.8 & 0.797 & 0.783 & 0.486 & 0.755 & 0.728 & 0.705 & 0.355 & 0.230 & 0.709 \\
 & SVD-LLM & 0.6 & 0.776 & 0.735 & 0.435 & 0.677 & 0.719 & 0.660 & 0.312 & 0.170 & 0.667 \\
 & SVD-LLM & 0.4 & 0.681 & 0.542 & 0.305 & 0.472 & 0.633 & 0.394 & 0.257 & 0.020 & 0.505 \\
 & SVD-LLM & 0.2 & 0.516 & 0.291 & 0.231 & 0.294 & 0.506 & 0.007 & 0.223 & 0.005 & 0.307 \\
 & Basis Sharing & 0.8 & 0.803 & 0.777 & 0.502 & 0.757 & 0.742 & 0.706 & 0.360 & 0.305 & 0.715 \\
 & Basis Sharing & 0.6 & 0.790 & 0.775 & 0.469 & 0.709 & 0.723 & 0.664 & 0.314 & 0.195 & 0.688 \\
 & Basis Sharing & 0.4 & 0.727 & 0.599 & 0.352 & 0.550 & 0.614 & 0.450 & 0.274 & 0.025 & 0.549 \\
 & Basis Sharing & 0.2 & 0.517 & 0.251 & 0.251 & 0.240 & 0.506 & 0.001 & 0.207 & 0.000 & 0.294 \\
\midrule
Llama-3-8B & dense & 1.0 & 0.805 & 0.790 & 0.531 & 0.796 & 0.738 & 0.750 & 0.401 & 0.435 & 0.735 \\
 & \ftc{} & 0.8 & 0.794 & 0.801 & 0.535 & 0.779 & 0.733 & 0.735 & 0.370 & 0.395 & 0.729 \\
 & \ftc{} & 0.6 & 0.788 & 0.786 & 0.501 & 0.766 & 0.740 & 0.717 & 0.326 & 0.290 & 0.716 \\
 & \ftc{} & 0.4 & 0.778 & 0.730 & 0.438 & 0.730 & 0.700 & 0.634 & 0.302 & 0.100 & 0.668 \\
 & \ftc{} & 0.2 & 0.702 & 0.522 & 0.308 & 0.521 & 0.596 & 0.282 & 0.241 & 0.020 & 0.488 \\
 & Seq-SVD & 0.6 & 0.739 & 0.702 & 0.422 & 0.684 & 0.716 & 0.590 & 0.345 & 0.085 & 0.642 \\
 & Seq-SVD & 0.4 & 0.683 & 0.467 & 0.315 & 0.518 & 0.641 & 0.436 & 0.257 & 0.035 & 0.510 \\
 & Seq-SVD & 0.2 & 0.541 & 0.312 & 0.234 & 0.329 & 0.541 & 0.113 & 0.221 & 0.005 & 0.345 \\
 & enh-LeSTD & 0.8 & 0.786 & 0.796 & 0.531 & 0.773 & 0.731 & 0.713 & 0.371 & 0.345 & 0.722 \\
 & enh-LeSTD & 0.6 & 0.782 & 0.784 & 0.486 & 0.754 & 0.716 & 0.641 & 0.330 & 0.195 & 0.694 \\
 & enh-LeSTD & 0.4 & 0.739 & 0.694 & 0.409 & 0.658 & 0.650 & 0.458 & 0.287 & 0.040 & 0.601 \\
 & enh-LeSTD & 0.2 & 0.588 & 0.365 & 0.249 & 0.358 & 0.536 & 0.044 & 0.226 & 0.005 & 0.357 \\
 & TLLM-gen & 0.8 & 0.767 & 0.760 & 0.483 & 0.727 & 0.715 & 0.647 & 0.313 & 0.070 & 0.683 \\
 & TLLM-gen & 0.6 & 0.731 & 0.657 & 0.394 & 0.641 & 0.660 & 0.498 & 0.267 & 0.035 & 0.597 \\
 & TLLM-gen & 0.4 & 0.671 & 0.472 & 0.289 & 0.489 & 0.584 & 0.175 & 0.241 & 0.025 & 0.447 \\
 & TLLM-gen & 0.2 & 0.565 & 0.328 & 0.235 & 0.314 & 0.507 & 0.015 & 0.215 & 0.010 & 0.327 \\
 & MPIFA & 0.8 & 0.793 & 0.771 & 0.506 & 0.760 & 0.725 & 0.683 & 0.375 & 0.360 & 0.706 \\
 & MPIFA & 0.6 & 0.741 & 0.711 & 0.441 & 0.664 & 0.709 & 0.570 & 0.342 & 0.005 & 0.639 \\
 & MPIFA & 0.4 & 0.622 & 0.421 & 0.278 & 0.439 & 0.608 & 0.323 & 0.242 & 0.020 & 0.448 \\
 & MPIFA & 0.2 & 0.517 & 0.277 & 0.222 & 0.277 & 0.522 & 0.019 & 0.199 & 0.000 & 0.306 \\
 & SVD-LLM & 0.8 & 0.770 & 0.738 & 0.461 & 0.733 & 0.724 & 0.589 & 0.357 & 0.040 & 0.669 \\
 & SVD-LLM & 0.6 & 0.720 & 0.626 & 0.381 & 0.613 & 0.682 & 0.427 & 0.317 & 0.020 & 0.575 \\
 & SVD-LLM & 0.4 & 0.610 & 0.389 & 0.266 & 0.403 & 0.578 & 0.215 & 0.243 & 0.040 & 0.410 \\
 & SVD-LLM & 0.2 & 0.523 & 0.279 & 0.242 & 0.277 & 0.501 & 0.027 & 0.221 & 0.030 & 0.308 \\
 & Basis Sharing & 0.8 & 0.791 & 0.720 & 0.458 & 0.732 & 0.715 & 0.619 & 0.343 & 0.330 & 0.672 \\
 & Basis Sharing & 0.6 & 0.742 & 0.637 & 0.394 & 0.680 & 0.686 & 0.550 & 0.340 & 0.045 & 0.615 \\
 & Basis Sharing & 0.4 & 0.653 & 0.448 & 0.294 & 0.498 & 0.626 & 0.325 & 0.254 & 0.025 & 0.474 \\
 & Basis Sharing & 0.2 & 0.527 & 0.288 & 0.234 & 0.278 & 0.535 & 0.027 & 0.219 & 0.015 & 0.315 \\
\midrule
Qwen2.5-7B & dense & 1.0 & 0.791 & 0.769 & 0.511 & 0.781 & 0.730 & 0.720 & 0.446 & 0.820 & 0.717 \\
 & \ftc{} & 0.8 & 0.796 & 0.797 & 0.511 & 0.780 & 0.714 & 0.690 & 0.439 & 0.780 & 0.715 \\
 & \ftc{} & 0.6 & 0.790 & 0.727 & 0.492 & 0.770 & 0.707 & 0.650 & 0.451 & 0.715 & 0.689 \\
 & \ftc{} & 0.4 & 0.785 & 0.732 & 0.486 & 0.742 & 0.676 & 0.535 & 0.395 & 0.445 & 0.659 \\
 & \ftc{} & 0.2 & 0.614 & 0.410 & 0.258 & 0.423 & 0.565 & 0.163 & 0.227 & 0.015 & 0.405 \\
 & Seq-SVD & 0.6 & 0.745 & 0.690 & 0.442 & 0.688 & 0.707 & 0.514 & 0.359 & 0.445 & 0.631 \\
 & Seq-SVD & 0.4 & 0.539 & 0.297 & 0.209 & 0.322 & 0.528 & 0.095 & 0.237 & 0.010 & 0.332 \\
 & Seq-SVD & 0.2 & 0.543 & 0.264 & 0.242 & 0.255 & 0.524 & 0.000 & 0.237 & 0.010 & 0.305 \\
 & enh-LeSTD & 0.8 & 0.787 & 0.777 & 0.497 & 0.767 & 0.709 & 0.639 & 0.426 & 0.705 & 0.696 \\
 & enh-LeSTD & 0.6 & 0.779 & 0.727 & 0.474 & 0.733 & 0.693 & 0.543 & 0.419 & 0.495 & 0.658 \\
 & enh-LeSTD & 0.4 & 0.673 & 0.533 & 0.322 & 0.551 & 0.622 & 0.240 & 0.306 & 0.015 & 0.490 \\
 & enh-LeSTD & 0.2 & 0.526 & 0.268 & 0.247 & 0.258 & 0.491 & 0.000 & 0.220 & 0.000 & 0.298 \\
 & TLLM-gen & 0.8 & 0.782 & 0.776 & 0.507 & 0.750 & 0.693 & 0.521 & 0.398 & 0.645 & 0.671 \\
 & TLLM-gen & 0.6 & 0.531 & 0.321 & 0.243 & 0.313 & 0.528 & 0.021 & 0.281 & 0.010 & 0.326 \\
 & TLLM-gen & 0.4 & 0.531 & 0.263 & 0.247 & 0.281 & 0.481 & 0.000 & 0.238 & 0.015 & 0.300 \\
 & TLLM-gen & 0.2 & 0.518 & 0.251 & 0.242 & 0.258 & 0.514 & 0.000 & 0.191 & 0.005 & 0.297 \\
 & MPIFA & 0.8 & 0.784 & 0.752 & 0.487 & 0.762 & 0.708 & 0.692 & 0.464 & 0.715 & 0.698 \\
 & MPIFA & 0.6 & 0.748 & 0.764 & 0.475 & 0.709 & 0.726 & 0.575 & 0.423 & 0.525 & 0.666 \\
 & MPIFA & 0.4 & 0.605 & 0.476 & 0.299 & 0.446 & 0.614 & 0.296 & 0.274 & 0.035 & 0.456 \\
 & MPIFA & 0.2 & 0.514 & 0.235 & 0.235 & 0.252 & 0.496 & 0.000 & 0.192 & 0.025 & 0.289 \\
 & SVD-LLM & 0.8 & 0.771 & 0.749 & 0.481 & 0.741 & 0.716 & 0.646 & 0.448 & 0.680 & 0.684 \\
 & SVD-LLM & 0.6 & 0.732 & 0.707 & 0.434 & 0.646 & 0.684 & 0.538 & 0.378 & 0.420 & 0.624 \\
 & SVD-LLM & 0.4 & 0.565 & 0.390 & 0.265 & 0.391 & 0.542 & 0.232 & 0.260 & 0.020 & 0.398 \\
 & SVD-LLM & 0.2 & 0.516 & 0.259 & 0.243 & 0.260 & 0.500 & 0.004 & 0.234 & 0.015 & 0.297 \\
 & Basis Sharing & 0.8 & 0.796 & 0.800 & 0.529 & 0.765 & 0.715 & 0.688 & 0.443 & 0.720 & 0.716 \\
 & Basis Sharing & 0.6 & 0.776 & 0.742 & 0.472 & 0.723 & 0.711 & 0.589 & 0.410 & 0.535 & 0.669 \\
 & Basis Sharing & 0.4 & 0.662 & 0.582 & 0.374 & 0.550 & 0.602 & 0.364 & 0.294 & 0.090 & 0.522 \\
 & Basis Sharing & 0.2 & 0.538 & 0.267 & 0.219 & 0.250 & 0.494 & 0.009 & 0.239 & 0.010 & 0.296 \\
\midrule
Qwen3-8B & dense & 1.0 & 0.786 & 0.801 & 0.561 & 0.774 & 0.724 & 0.704 & 0.562 & 0.855 & 0.725 \\
 & \ftc{} & 0.8 & 0.788 & 0.832 & 0.583 & 0.763 & 0.735 & 0.664 & 0.563 & 0.765 & 0.728 \\
 & \ftc{} & 0.6 & 0.781 & 0.793 & 0.564 & 0.750 & 0.715 & 0.640 & 0.515 & 0.735 & 0.707 \\
 & \ftc{} & 0.4 & 0.730 & 0.641 & 0.441 & 0.712 & 0.670 & 0.553 & 0.316 & 0.105 & 0.624 \\
 & \ftc{} & 0.2 & 0.690 & 0.550 & 0.324 & 0.550 & 0.582 & 0.305 & 0.247 & 0.005 & 0.500 \\
 & Seq-SVD & 0.6 & 0.765 & 0.712 & 0.487 & 0.718 & 0.699 & 0.627 & 0.423 & 0.455 & 0.668 \\
 & Seq-SVD & 0.4 & 0.707 & 0.567 & 0.373 & 0.606 & 0.642 & 0.472 & 0.284 & 0.085 & 0.561 \\
 & Seq-SVD & 0.2 & 0.557 & 0.320 & 0.209 & 0.305 & 0.534 & 0.129 & 0.245 & 0.005 & 0.342 \\
 & enh-LeSTD & 0.8 & 0.789 & 0.831 & 0.590 & 0.753 & 0.718 & 0.617 & 0.547 & 0.790 & 0.716 \\
 & enh-LeSTD & 0.6 & 0.773 & 0.760 & 0.493 & 0.684 & 0.664 & 0.489 & 0.454 & 0.540 & 0.644 \\
 & enh-LeSTD & 0.4 & 0.724 & 0.609 & 0.388 & 0.558 & 0.604 & 0.294 & 0.307 & 0.070 & 0.529 \\
 & enh-LeSTD & 0.2 & 0.555 & 0.348 & 0.238 & 0.305 & 0.514 & 0.016 & 0.215 & 0.005 & 0.329 \\
 & TLLM-gen & 0.8 & 0.777 & 0.761 & 0.499 & 0.706 & 0.700 & 0.519 & 0.468 & 0.635 & 0.660 \\
 & TLLM-gen & 0.6 & 0.749 & 0.671 & 0.444 & 0.629 & 0.647 & 0.373 & 0.393 & 0.235 & 0.586 \\
 & TLLM-gen & 0.4 & 0.663 & 0.495 & 0.320 & 0.454 & 0.550 & 0.109 & 0.286 & 0.010 & 0.432 \\
 & TLLM-gen & 0.2 & 0.532 & 0.297 & 0.215 & 0.282 & 0.500 & 0.001 & 0.210 & 0.000 & 0.304 \\
 & MPIFA & 0.8 & 0.791 & 0.773 & 0.570 & 0.780 & 0.714 & 0.626 & 0.484 & 0.695 & 0.709 \\
 & MPIFA & 0.6 & 0.773 & 0.722 & 0.505 & 0.740 & 0.714 & 0.564 & 0.450 & 0.440 & 0.670 \\
 & MPIFA & 0.4 & 0.684 & 0.531 & 0.330 & 0.536 & 0.644 & 0.406 & 0.279 & 0.080 & 0.522 \\
 & MPIFA & 0.2 & 0.554 & 0.333 & 0.217 & 0.311 & 0.533 & 0.199 & 0.225 & 0.000 & 0.358 \\
 & SVD-LLM & 0.8 & 0.777 & 0.752 & 0.529 & 0.762 & 0.715 & 0.542 & 0.436 & 0.335 & 0.679 \\
 & SVD-LLM & 0.6 & 0.750 & 0.577 & 0.416 & 0.690 & 0.688 & 0.488 & 0.373 & 0.200 & 0.601 \\
 & SVD-LLM & 0.4 & 0.624 & 0.446 & 0.255 & 0.393 & 0.555 & 0.278 & 0.246 & 0.010 & 0.425 \\
 & SVD-LLM & 0.2 & 0.520 & 0.302 & 0.214 & 0.276 & 0.511 & 0.106 & 0.226 & 0.005 & 0.322 \\
 & Basis Sharing & 0.8 & 0.774 & 0.769 & 0.566 & 0.765 & 0.716 & 0.561 & 0.458 & 0.430 & 0.692 \\
 & Basis Sharing & 0.6 & 0.775 & 0.746 & 0.531 & 0.724 & 0.707 & 0.482 & 0.406 & 0.200 & 0.661 \\
 & Basis Sharing & 0.4 & 0.737 & 0.587 & 0.402 & 0.632 & 0.638 & 0.369 & 0.330 & 0.045 & 0.561 \\
 & Basis Sharing & 0.2 & 0.544 & 0.289 & 0.207 & 0.306 & 0.529 & 0.137 & 0.239 & 0.005 & 0.335 \\
\midrule
Qwen3-32B & dense & 1.0 & 0.802 & 0.829 & 0.608 & 0.818 & 0.729 & 0.671 & 0.611 & 0.885 & 0.743 \\
 & \ftc{} & 0.6 & 0.801 & 0.815 & 0.594 & 0.811 & 0.723 & 0.656 & 0.536 & 0.770 & 0.733 \\
 & \ftc{} & 0.4 & 0.799 & 0.812 & 0.617 & 0.795 & 0.739 & 0.635 & 0.487 & 0.750 & 0.733 \\
 & \ftc{} & 0.2 & 0.782 & 0.777 & 0.556 & 0.727 & 0.696 & 0.489 & 0.359 & 0.280 & 0.671 \\
 & Seq-SVD & 0.6 & 0.784 & 0.809 & 0.607 & 0.786 & 0.728 & 0.666 & 0.483 & 0.635 & 0.730 \\
 & Seq-SVD & 0.4 & 0.768 & 0.762 & 0.536 & 0.728 & 0.714 & 0.565 & 0.380 & 0.545 & 0.679 \\
 & Seq-SVD & 0.2 & 0.582 & 0.380 & 0.253 & 0.370 & 0.530 & 0.134 & 0.233 & 0.000 & 0.375 \\
 & enh-LeSTD & 0.6 & 0.799 & 0.811 & 0.596 & 0.784 & 0.727 & 0.587 & 0.532 & 0.765 & 0.717 \\
 & enh-LeSTD & 0.4 & 0.786 & 0.784 & 0.595 & 0.751 & 0.734 & 0.441 & 0.469 & 0.510 & 0.682 \\
 & enh-LeSTD & 0.2 & 0.685 & 0.494 & 0.356 & 0.542 & 0.593 & 0.092 & 0.281 & 0.015 & 0.460 \\
 & TLLM-gen & 0.6 & 0.795 & 0.788 & 0.580 & 0.767 & 0.728 & 0.463 & 0.505 & 0.700 & 0.687 \\
 & TLLM-gen & 0.4 & 0.785 & 0.718 & 0.513 & 0.708 & 0.706 & 0.278 & 0.409 & 0.210 & 0.618 \\
 & TLLM-gen & 0.2 & 0.594 & 0.358 & 0.268 & 0.366 & 0.530 & 0.017 & 0.228 & 0.000 & 0.355 \\
 & MPIFA & 0.6 & 0.783 & 0.788 & 0.632 & 0.779 & 0.724 & 0.628 & 0.475 & 0.715 & 0.722 \\
 & MPIFA & 0.4 & 0.734 & 0.711 & 0.501 & 0.657 & 0.665 & 0.504 & 0.370 & 0.405 & 0.629 \\
 & MPIFA & 0.2 & 0.594 & 0.335 & 0.246 & 0.341 & 0.517 & 0.200 & 0.230 & 0.015 & 0.372 \\
 & SVD-LLM & 0.6 & 0.765 & 0.745 & 0.566 & 0.751 & 0.698 & 0.579 & 0.426 & 0.665 & 0.684 \\
 & SVD-LLM & 0.4 & 0.708 & 0.587 & 0.380 & 0.523 & 0.605 & 0.348 & 0.293 & 0.035 & 0.525 \\
 & SVD-LLM & 0.2 & 0.545 & 0.303 & 0.218 & 0.287 & 0.521 & 0.135 & 0.242 & 0.000 & 0.335 \\
 & Basis Sharing & 0.6 & 0.781 & 0.753 & 0.579 & 0.771 & 0.723 & 0.600 & 0.479 & 0.600 & 0.701 \\
 & Basis Sharing & 0.4 & 0.761 & 0.741 & 0.534 & 0.720 & 0.683 & 0.504 & 0.358 & 0.440 & 0.657 \\
 & Basis Sharing & 0.2 & 0.601 & 0.363 & 0.242 & 0.343 & 0.501 & 0.163 & 0.241 & 0.010 & 0.369 \\
\midrule
Qwen3.5-9B & dense & 1.0 & 0.794 & 0.776 & 0.565 & 0.770 & 0.734 & 0.696 & 0.553 & 0.885 & 0.723 \\
 & \ftc{} & 0.8 & 0.794 & 0.833 & 0.602 & 0.748 & 0.716 & 0.671 & 0.512 & 0.785 & 0.727 \\
 & \ftc{} & 0.6 & 0.755 & 0.822 & 0.550 & 0.681 & 0.705 & 0.625 & 0.421 & 0.580 & 0.690 \\

==> tables/a4_accounting.tex <==
GPT-J-6B & 0.8 & 0.800 & 0.846 & 31.1\% & 4.8\% \\
 & 0.6 & 0.600 & 0.639 & 31.1\% & 11.2\% \\
 & 0.4 & 0.400 & 0.429 & 31.1\% & 17.7\% \\
 & 0.2 & 0.200 & 0.215 & 31.1\% & 24.4\% \\
\midrule
Llama-2-13B & 0.8 & 0.800 & 0.847 & 32.2\% & 4.9\% \\
 & 0.6 & 0.600 & 0.637 & 32.2\% & 11.7\% \\
 & 0.4 & 0.400 & 0.429 & 32.2\% & 18.4\% \\
 & 0.2 & 0.200 & 0.217 & 32.2\% & 25.2\% \\
\midrule
Mistral-7B & 0.8 & 0.797 & 0.820 & 18.5\% & 3.3\% \\
 & 0.6 & 0.600 & 0.619 & 18.5\% & 7.1\% \\
 & 0.4 & 0.400 & 0.414 & 18.5\% & 10.9\% \\
 & 0.2 & 0.200 & 0.207 & 18.5\% & 14.7\% \\
\midrule
Llama-3-8B & 0.8 & 0.800 & 0.823 & 16.7\% & 3.0\% \\
 & 0.6 & 0.600 & 0.619 & 16.7\% & 6.4\% \\
 & 0.4 & 0.400 & 0.414 & 16.7\% & 9.8\% \\
 & 0.2 & 0.200 & 0.207 & 16.7\% & 13.3\% \\
\midrule
Qwen2.5-7B & 0.8 & 0.800 & 0.820 & 10.8\% & 1.9\% \\
 & 0.6 & 0.600 & 0.615 & 10.8\% & 4.2\% \\
 & 0.4 & 0.400 & 0.412 & 10.8\% & 6.3\% \\
 & 0.2 & 0.200 & 0.206 & 10.8\% & 8.6\% \\
\midrule
Qwen3-8B & 0.8 & 0.800 & 0.824 & 18.4\% & 3.3\% \\
 & 0.6 & 0.600 & 0.619 & 18.4\% & 7.0\% \\
 & 0.4 & 0.400 & 0.414 & 18.4\% & 10.8\% \\
 & 0.2 & 0.200 & 0.207 & 18.4\% & 14.6\% \\
\midrule

==> tables/abl_chain.tex <==
Llama-3 w/o whitening & 26.408 & 11.723 & +125.3\% \\
Llama-3 w/o teacher & 11.420 & 11.723 & -2.6\% \\
Qwen3 w/o whitening & 31.761 & 12.085 & +162.8\% \\
Qwen3 w/o teacher & 15.105 & 12.085 & +25.0\% \\
Mistral w/o whitening & 14.891 & 9.738 & +52.9\% \\
Mistral w/o seq.\ streams & 17.885 & 9.738 & +83.7\% \\

==> tables/abl_nojoint.tex <==
Mistral 0.6 & 5.707 & 5.507 & +3.6\% \\
Mistral 0.2 & 12.536 & 9.738 & +28.7\% \\
Llama-3 0.6 & 7.143 & 6.613 & +8.0\% \\
Llama-3 0.2 & 24.316 & 11.723 & +107.4\% \\
Qwen2.5 0.6 & 8.216 & 7.312 & +12.4\% \\
Qwen2.5 0.2 & 100.750 & 47.999 & +109.9\% \\
Qwen3 0.6 & 7.935 & 7.764 & +2.2\% \\
Qwen3 0.2 & 21.854 & 12.085 & +80.8\% \\

==> tables/t1_main_ppl.tex <==
\multirow{2}{*}{GPT-J-6B (8.86)} & 0.6 & \cellcolor{best}\textbf{9.30} & 9.47 & 9.93 & 9.68 & 9.46 & 10.26 & 10.16 \\
 & 0.2 & \cellcolor{best}\textbf{13.60} & 14.84 & 17.47 & 19.22 & 17.24 & 25.04 & 23.02 \\
\midrule
\multirow{2}{*}{Llama-2-13B (4.89)} & 0.6 & \cellcolor{best}\textbf{5.11} & 5.27 & 5.13 & 5.52 & 5.26 & 5.68 & 5.57 \\
 & 0.2 & \cellcolor{best}\textbf{7.52} & 9.00 & 9.79 & 13.01 & 10.21 & 14.20 & 12.77 \\
\midrule
\multirow{2}{*}{Mistral-7B (5.32)} & 0.6 & \cellcolor{best}\textbf{5.44} & 5.69 & 5.58 & 6.07 & 5.63 & 5.92 & 5.75 \\
 & 0.2 & \cellcolor{best}\textbf{7.33} & 12.10 & 146.31 & 18.41 & 15.92 & 25.40 & 16.18 \\
\midrule
\multirow{2}{*}{Llama-3-8B (6.14)} & 0.6 & \cellcolor{best}\textbf{6.64} & 7.03 & 6.82 & 8.70 & 7.26 & 8.02 & 7.60 \\
 & 0.2 & \cellcolor{best}\textbf{10.44} & 19.46 & 20.84 & 29.85 & 27.02 & 48.09 & 35.60 \\
\midrule
\multirow{2}{*}{Qwen2.5-7B (6.85)} & 0.6 & \cellcolor{best}\textbf{7.20} & 7.98 & 7.76 & 34.10 & 7.84 & 8.56 & 7.82 \\
 & 0.2 & \cellcolor{best}\textbf{12.55} & 150.93 & 106.59 & 188.22 & 7791 & 255.23 & 140.65 \\
\midrule
\multirow{2}{*}{Qwen3-8B (7.00)} & 0.6 & \cellcolor{best}\textbf{7.36} & 7.65 & 8.20 & 9.12 & 8.17 & 9.24 & 9.18 \\
 & 0.2 & \cellcolor{best}\textbf{10.70} & 23.66 & 27.08 & 45.45 & 22.23 & 75.77 & 46.68 \\
\midrule
\multirow{2}{*}{Qwen3-32B (7.61)} & 0.6 & \cellcolor{best}\textbf{7.77} & 7.98 & 7.84 & 8.56 & 8.40 & 9.23 & 8.70 \\
 & 0.2 & \cellcolor{best}\textbf{9.22} & 22.97 & 15.23 & 29.71 & 26.75 & 66.29 & 29.63 \\

==> tables/t4_throughput.tex <==
MHA (GPT-J-6B) & 64 & 0.6 & 1.08$\times$ & 0.15$\times$ \\
 & 64 & 0.2 & 1.91$\times$ & 0.14$\times$ \\
 & 2048 & 0.6 & 1.12$\times$ & 0.79$\times$ \\
 & 2048 & 0.2 & 2.22$\times$ & 1.01$\times$ \\
 & 8192 & 0.6 & 1.05$\times$ & 1.05$\times$ \\
 & 8192 & 0.2 & 2.53$\times$ & 2.18$\times$ \\
\midrule
GQA (Llama-3 / Qwen3) & 64 & 0.6 & 0.84$\times$ & 0.08$\times$ \\
 & 64 & 0.2 & 1.24$\times$ & 0.08$\times$ \\
 & 2048 & 0.6 & 1.74$\times$ & 0.62$\times$ \\
 & 2048 & 0.2 & 3.03$\times$ & 0.67$\times$ \\
 & 8192 & 0.6 & 1.68$\times$ & 1.47$\times$ \\
 & 8192 & 0.2 & 3.22$\times$ & 1.86$\times$ \\
\midrule
Hybrid (Qwen3.5, DeltaNet) & 64 & 0.6 & 0.97$\times$ & 0.09$\times$ \\
 & 64 & 0.2 & 1.50$\times$ & 0.09$\times$ \\
 & 2048 & 0.6 & 1.82$\times$ & 0.75$\times$ \\
 & 2048 & 0.2 & 3.20$\times$ & 0.82$\times$ \\
 & 8192 & 0.6 & 1.66$\times$ & 1.57$\times$ \\
 & 8192 & 0.2 & 3.27$\times$ & 2.11$\times$ \\

==> tables/t_layer_align.tex <==

Mistral-7B
& dense (ms)
& 0.53 & 0.58 & 0.61 & 1.02 & 5.83 & 25.27 \\
& unaligned ranks
& 1.17 & 1.00 & 0.90 & 0.91 & 0.90 & 0.91 \\
& ranks aligned to 8
& 1.05 & 1.07 & 1.03 & 1.00 & 0.98 & 0.98 \\
& deployable structured
& 1.01 & 1.03 & 0.86 & 0.97 & 0.95 & 0.94 \\
\midrule

Llama-3-8B
& dense (ms)
& 0.53 & 0.58 & 0.61 & 1.03 & 5.92 & 25.60 \\
& unaligned ranks
& 1.04 & 1.00 & 0.91 & 0.92 & 0.92 & 0.92 \\
& ranks aligned to 8
& 1.04 & 1.06 & 1.02 & 1.00 & 0.99 & 1.00 \\
& deployable structured
& 1.00 & 1.03 & 0.98 & 0.98 & 0.96 & 0.96 \\
\midrule

Qwen3-8B
& dense (ms)
& 0.52 & 0.56 & 0.60 & 0.95 & 5.71 & 24.62 \\
& unaligned ranks
& 1.07 & 0.80 & 0.77 & 0.71 & 0.75 & 0.76 \\
& ranks aligned to 8
& 1.08 & 1.06 & 1.03 & 0.97 & 1.01 & 1.00 \\
& deployable structured
& 1.04 & 1.02 & 1.01 & 0.97 & 0.97 & 0.96 \\
\midrule

Qwen3-32B
& dense (ms)
& 0.98 & 1.04 & 1.12 & 2.00 & 12.35 & 53.77 \\
& unaligned ranks
& 1.18 & 0.91 & 0.82 & 0.81 & 0.74 & 0.73 \\
& ranks aligned to 8
& 1.20 & 1.20 & 1.15 & 1.03 & 1.02 & 1.02 \\
& deployable structured
& 1.12 & 1.10 & 1.08 & 1.00 & 0.96 & 0.94 \\
